FEC for Lower In-Order Delivery Delay in Packet Networks

We consider use of FEC to reduce in-order delivery delay over packet erasure channels. We propose a class of streaming codes that is capacity achieving and provides a superior throughput-delay trade-off compared to block codes by introducing flexibility in where and when redundancy is placed. This flexibility results in significantly lower in-order delay for a given throughput for a wide range of network scenarios. Furthermore, a major contribution of this paper is the combination of queuing and coding theory to analyze the code's performance. Finally, we present simulation and experimental results illustrating the code's benefits.

==> group.tex <==

In this section, we assume that instead of one coded packet after each $l-1$ information packets, we put $c$ coded packets at the end of each $l_g-c$ information packets. We assume that these $c$ coded packets can recover up to $c$ erasures that happened prior to them. In order to compare the delay behavior of this scheme with the original scheme, we assume that $l_g = c l$ which means that the coding rate of both schemes are identical and equal to $ 1 - \frac{1}{l} = 1 - \frac {c}{l_g}.$ 

Following the same steps as before, we define the process $S_g$ as the busy period of the decoding operation.  Unfortunately, we have not been able to extend the same proof technique to this case. However, we use theorems in the lattice theory to find the following formula for the distribution of $S_g$, when there are $c$ coded packets in each interval $l_g$:

\begin{theorem}[Busy Time for Group Coded Packets]\label{maingeniedetgroup}
In an erasure channel with erasure probability $\epsilon$, suppose we insert $c$ coded packets in between every $l_g-c$ information packets.  Assume that each coded packet can help us to recover from $c$ erasures.  
%Suppose an erasure happens and the decoding procedure starts at time $t=0$.  Suppose $S=k$ denotes the $k$-th coding packet that will put an end to a decoding procedure at time $t= k l$.   
We have:

%\begin{itemize}
\noindent $I$.  For all values of $\epsilon$ and $l_g$ such that $l_g \epsilon < c$, the mean of the probability distribution of $S$ exists and is finite. 
%
%\emph{II}.
\begin{flalign}
\text{II.}
\quad S_g(0) & = (1 - \epsilon)^{l_g-c} \\
S_g(k) & = \sum_{p=0}^{c-1} NP(l,c,k,p)  \epsilon^{kc-p}  (1-\epsilon)^{kl-kc+p}, 
\end{flalign}
%
where the exact value of $NP(l,c,k,p)$ is computed in the proof of the theorem. 
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

In Fig. \ref{fig:groupcode}, through simulations, it is shown that the average in order delivery delay per information packet is an increasing function of $c$, the number of coded packets at the end of each interval.  \textbf{**more discussion to be added.}

\begin{figure}
\centering
\includegraphics[width=0.99\columnwidth]{figures/delaygroup.pdf}
\caption{Average in order delivery delay per information packet, $c$ is the number of coded packets at the end of each interval, $\epsilon = 0.1$.}\label{fig:groupcode}
\end{figure}
